Hard negative sampling in hyperedge prediction

Hypergraph, which allows each hyperedge to encompass an arbitrary number of nodes, is a powerful tool for modeling multi-entity interactions. Hyperedge prediction is a fundamental task that aims to predict future hyperedges or identify existent but unobserved hyperedges based on those observed. In link prediction for simple graphs, most observed links are treated as positive samples, while all unobserved links are considered as negative samples. However, this full-sampling strategy is impractical for hyperedge prediction, due to the number of unobserved hyperedges in a hypergraph significantly exceeds the number of observed ones. Therefore, one has to utilize some negative sampling methods to generate negative samples, ensuring their quantity is comparable to that of positive samples. In current hyperedge prediction, randomly selecting negative samples is a routine practice. But through experimental analysis, we discover a critical limitation of random selecting that the generated negative samples are too easily distinguishable from positive samples. This leads to premature convergence of the model and reduces the accuracy of prediction. To overcome this issue, we propose a novel method to generate negative samples, named as hard negative sampling (HNS). Unlike traditional methods that construct negative hyperedges by selecting node sets from the original hypergraph, HNS directly synthesizes negative samples in the hyperedge embedding space, thereby generating more challenging and informative negative samples. Our results demonstrate that HNS significantly enhances both accuracy and robustness of the prediction. Moreover, as a plug-and-play technique, HNS can be easily applied in the training of various hyperedge prediction models based on representation learning.

==> tables/cns_experiment.tex <==
\begin{table}[ht]
	\centering
	\scriptsize
	% \setlength{\tabcolsep}{2pt}
	\begin{tabularx}{0.7\linewidth}{lcccccccr} 
		\toprule
		\Th{Dataset} & \mc{2}{\Th{CiteSeer}} & \mc{2}{\Th{Cora}} & \mc{2}{Pubmed} & \mc{2}{NDC-Class}  \\ 
		& AP & AUC & AP & AUC & AP & AUC & AP & AUC  \\ 
		\midrule
		HGNN      & 0.4637 & 0.4253 & 0.4808 & 0.4556 & 0.4653 & 0.418 & 0.4911 & 0.4913 \\
		HGNN(HNS)  &  0.5004 & 0.4508 & 0.5151 & 0.4985 & 0.4827 & 0.4486 & 0.5566 & 0.5649 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0367} & \gp{+0.0255} & \gp{+0.0343} & \gp{+0.0429} & \gp{+0.0174} & \gp{+0.0306} & \gp{+0.0655} & \gp{+0.0736} \\
		\midrule
		HNHN       & 0.4351 & 0.3729 & 0.4788 & 0.452 & 0.4634 & 0.4188 & 0.473 & 0.4487 \\
		HNHN(HNS)    & 0.5009 & 0.4753 & 0.5202 & 0.4712 & 0.4734 & 0.4404 & 0.6254 & 0.5571 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0658} & \gp{+0.1024} & \gp{+0.0414} & \gp{+0.0192} & \gp{+0.01} & \gp{+0.0216} & \gp{+0.1524} & \gp{+0.1084} \\
		\midrule
		NHP      & 0.4569 & 0.4032 & 0.5022 & 0.4613 & 0.4696 & 0.4222 & 0.4955 & 0.4905 \\
		NHP(HNS) & 0.4703 & 0.4462 & 0.5087 & 0.471  & 0.5264 & 0.5027 & 0.5213 & 0.5364 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0134} & \gp{+0.043} & \gp{+0.0065} & \gp{+0.0097} & \gp{+0.0568} & \gp{+0.0805} & \gp{+0.0258} & \gp{+0.0459} \\
		\midrule
		HGNNP      & 0.4699 & 0.3877 & 0.4643 & 0.4289 & 0.4541 & 0.4169 & 0.5    & 0.502 \\
		HGNNP(HNS) & 0.473  & 0.4269 & 0.4929 & 0.4777 & 0.4608 & 0.4189 & 0.6661 & 0.598 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0031} & \gp{+0.0392} & \gp{+0.0286} & \gp{+0.0488} & \gp{+0.0067} & \gp{+0.002} & \gp{+0.1661} & \gp{+0.096} \\
		\bottomrule
	\end{tabularx}
    \begin{tabularx}{0.7\linewidth}{lcccccr} 
		\toprule
		\Th{Dataset} & \mc{2}{Email-Enron} & \mc{2}{Human-Disease} & \mc{2}{Plant-Pollinator} \\ 
		& AP & AUC & AP & AUC & AP & AUC \\ 
		\midrule
		HGNN       & 0.6296 & 0.6663 & 0.4691 & 0.3779 & 0.5567 & 0.5978 \\
		HGNN(HNS)  & 0.6757 & 0.6791 & 0.6322 & 0.6157 & 0.5645 & 0.6131 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0461} & \gp{+0.0128} & \gp{+0.1631} & \gp{+0.2378} & \gp{+0.0078} & \gp{+0.0153} \\
		\midrule
		HNHN        & 0.6066 & 0.6422 & 0.4589 & 0.3466 & 0.5392 & 0.5844 \\
		HNHN(HNS)   & 0.6545 & 0.6691 & 0.5901 & 0.5 & 0.5396 & 0.5837 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0479} & \gp{+0.0269} & \gp{+0.1312} & \gp{+0.1534} & \gp{+0.0004} & \gn{-0.0007} \\
		\midrule
		NHP      & 0.6081 & 0.6149 & 0.4868 & 0.3935 & 0.5542 & 0.5697 \\
		NHP(HNS) & 0.6252 & 0.6312 & 0.6051 & 0.5854 & 0.57   & 0.5708 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0171} & \gp{+0.0163} & \gp{+0.1183} & \gp{+0.1919} & \gp{+0.0158} & \gp{+0.0011} \\
		\midrule
		HGNNP      & 0.6366 & 0.6692 & 0.4534 & 0.3613 & 0.5447 & 0.5915 \\
		HGNNP(HNS) & 0.6675 & 0.6813 & 0.4651 & 0.3724 & 0.5317 & 0.5865 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0309} & \gp{+0.0121} & \gp{+0.0117} & \gp{+0.0111} & \gn{-0.013} & \gn{-0.005} \\
		\bottomrule
	\end{tabularx}
	\caption{采用CNS方式生成测试集的负样本, 不同模型的分类在不同的负采样方法下的准确率对比. 在每种超边预测方法下, 第一行代表使用CNS方法获取负样本, 第二行代表使用HNS方法获取负样本所得到的结果.}
	\label{cns_experiment_table}
\end{table}

==> tables/main_experiment_table.tex <==
\begin{table}[ht]
	\centering
	\scriptsize
	% \setlength{\tabcolsep}{3pt}
    \begin{tabularx}{\linewidth}{l*{7}{>{\centering\arraybackslash}X}}
	% \begin{tabularx}{0.7\linewidth}{lcccccccr} 
		\toprule
		\Th{Dataset} & \mc{2}{\Th{CiteSeer}}  & \mc{2}{\Th{Cora}}& \mc{2}{Pubmed} & \mc{2}{NDC-Class} \\
		& AP & AUC & AP & AUC & AP & AUC & AP & AUC	\\
		\midrule
		HGNN & 0.9361 & 0.9333 & 0.8955 & 0.8899 & 0.9506 & 0.9502 & 0.9821 & 0.9807  \\
		HGNN(HNS) & 0.9577 & 0.9597 & 0.9623 & 0.9537 & 0.9649 & 0.9661 & 0.9870 & 0.9846 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0216} & \gp{+0.0264} & \gp{+0.0668} & \gp{+0.0638} & \gp{+0.0143} & \gp{+0.0159} & \gp{+0.0068} & \gp{+0.0070} \\
		\midrule
		HNHN & 0.9555 & 0.9573 & 0.9298 & 0.9342 & 0.9366 & 0.9415 & 0.9818 & 0.9803 \\
		HNHN(HNS) & 0.9633 & 0.9601 & 0.9459 & 0.9451 & 0.9472 & 0.9426 & 0.9829 & 0.9817 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0078} & \gp{+0.0028} & \gp{+0.0161} & \gp{+0.0109} & \gp{+0.0106} & \gp{+0.0011} & \gp{+0.0011} & \gp{+0.0014} \\
		\midrule
		NHP & 0.9653 & 0.9589 & 0.9156 & 0.9137 & 0.9469 & 0.9414 & 0.9876 & 0.9876 \\
		NHP(HNS) & 0.9721 & 0.9638 & 0.9467 & 0.9359 & 0.9473 & 0.9415 & 0.9879 & 0.9877 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0068} & \gp{+0.0049} & \gp{+0.0311} & \gp{+0.0222} & \gp{+0.0004} & \gp{+0.0001} & \gp{+0.0003} & \gp{+0.0001} \\
		\midrule
		HGNNP         & 0.9748 & 0.9719 & 0.9146 & 0.9172 & 0.934  & 0.9406  & 0.9871  & 0.9863 \\
		HGNNP(HNS)    & 0.9855 & 0.9828 & 0.9456 & 0.9308 & 0.9409 & 0.9354  & 0.9939  & 0.9933 \\
		\rowcolor{LightCyan}
		\textbf{Gain} &  \gp{+0.0107} & \gp{+0.0109} & \gp{+0.0310}  & \gp{+0.0136} & \gp{+0.0069} & \gn{-0.0052} & \gp{+0.0068} & \gp{+0.0070} \\
		\bottomrule
	\end{tabularx}
    \begin{tabularx}{0.7\linewidth}{lcccccr} 
		\toprule
		\Th{Dataset} & \mc{2}{Email-Enron} & \mc{2}{Human-Disease} & \mc{2}{Plant-Pollinator} \\
		& AP & AUC & AP & AUC & AP & AUC \\
		\midrule
		HGNN & 0.9724 & 0.9775 & 0.963 & 0.9743 & 0.9905 & 0.9909  \\
		HGNN(HNS) & 0.9735 & 0.9753 & 0.9774 & 0.9807 & 0.994 & 0.9938  \\
		\rowcolor{LightCyan}
		\tb{Gain} &\gp{+0.0011} & \gn{-0.0022} & \gp{+0.0144} & \gp{+0.0064} & \gp{+0.0035} & \gp{+0.0029} \\
		\midrule
		HNHN & 0.9854 & 0.9842 & 0.9334 & 0.966 & 0.9843 & 0.9859 \\
		HNHN(HNS) & 0.9862 & 0.9852 & 0.9761 & 0.9798 & 0.9847 & 0.9863	\\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0008} & \gp{+0.0010} & \gp{+0.0427} & \gp{+0.0138} & \gp{+0.0004} & \gp{+0.0004} \\
		\midrule
		NHP & 0.9665 & 0.9750 & 0.8892 & 0.9238 & 0.984 & 0.9859 \\
		NHP(HNS) & 0.9798 & 0.9779 & 0.9167 & 0.9256 & 0.9856 & 0.9867 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0133} & \gp{+0.0029} & \gp{+0.0275} & \gp{+0.0018} & \gp{+0.0016} & \gp{+0.0008}  \\
		\midrule
		HGNNP        & 0.9842 & 0.9839 & 0.9421 & 0.9467 & 0.9594 & 0.9716  \\
		HGNNP(HNS)   & 0.9842 & 0.9834 & 0.9504 & 0.955 & 0.9639 & 0.9726  \\
		\rowcolor{LightCyan}
		\textbf{Gain} & 0      & \gn{-0.0005} & \gp{+0.0083} & \gp{+0.0083} & \gp{+0.0045} & \gp{+0.001} \\
		\bottomrule
	\end{tabularx}
	\caption{不同超图链路预测模型在7个数据集上使用随机负采样与改进负样本生成方法的性能对比.在每种超边预测方法下, VMNS和VCNS分别为MNS和CNS用于验证集上的表现，而TMNS和TCNS为MNS和CNS用于训练集上的表现}
	\label{main_experiment_table}
\end{table}

==> tables/main_experiment_table2.tex <==
\begin{table}[ht]
	\centering
	\scriptsize
	\setlength{\tabcolsep}{4.5pt}
	\begin{tabularx}{\linewidth}{lcccccccccccccr} 
		\toprule
		\Th{Dataset} & \mc{2}{\Th{CiteSeer}} & \mc{2}{\Th{Cora}} & \mc{2}{Pubmed} & \mc{2}{NDC-Class}  & \mc{2}{Email-Enron} & \mc{2}{Human-Disease} & \mc{2}{Plant-Pollinator} \\  
		& AP & AUC & AP & AUC & AP & AUC & AP & AUC  & AP & AUC & AP & AUC & AP & AUC \\ 
		\midrule
		HGNN(SNS)     & 0.9361 & 0.9333 & 0.8955 & 0.8899 & \underline{0.9506} & \underline{0.9502} & 0.9821 & 0.9807 & \underline{0.9724} & \textbf{0.9775} & 0.9630 & 0.9743 & 0.9905 & 0.9909 \\
		HGNN(VMNS)    & \underline{0.9558} & \underline{0.9558 }& 0.8718 & 0.8648 & 0.9415 & 0.9374 & 0.9749 & 0.9719 & \textbf{0.9735} & \underline{0.9767} & 0.8680 & 0.8696 & \underline{0.9908} & \underline{0.9914} \\
		HGNN(VCNS)    & 0.9239 & 0.9284 & 0.8593 & 0.8567 & 0.9313 & 0.9446 & 0.9749 & 0.9719 & \textbf{0.9735} & \underline{0.9767} & \underline{0.9767} & \underline{0.9761} & \underline{0.9908} & \underline{0.9914} \\
        HGNN(TMNS)    & 0.8708 & 0.8434 & \underline{0.9353} & \underline{0.9221} & 0.7724 & 0.7497 & \underline{0.9844} & \underline{0.9818} & 0.9634 & 0.9628 & 0.9701 & 0.9697 & 0.9877 & 0.9891 \\
        HGNN(TCNS)    & 0.6955 & 0.5887 & 0.5338 & 0.4330 & 0.4207 & 0.3265 & 0.8436 & 0.8153 & 0.8489 & 0.8367 & 0.6801 & 0.6097 & 0.5930 & 0.6869 \\
		HGNN(HNS)     & \textbf{0.9577} & \textbf{0.9597} & \textbf{0.9623} & \textbf{0.9537} & \textbf{0.9649} & \textbf{0.9661} & \textbf{0.9870} & \textbf{0.9846} & \textbf{0.9735} & 0.9753 & \textbf{0.9774} & \textbf{0.9807} & \textbf{0.9940} & \textbf{0.9938} \\	
		\midrule
		HNHN(SNS)     & 0.9555 & \underline{0.9573} & \underline{0.9298} & \underline{0.9342} & 0.9366 & \underline{0.9415} & 0.9818 & 0.9803 & \underline{0.9854 }& \underline{0.9842} & 0.9334 & 0.9660 & \underline{0.9843} & \underline{0.9859} \\
		HNHN(VMNS)    & \underline{0.9600} & 0.9540 & 0.9243 & 0.8977 & \underline{0.9420} & 0.9367 & \underline{0.9877} & \underline{0.9862} &0.9660  & 0.9619 & 0.9535 & 0.9541 & 0.9690 & 0.9748 \\
		HNHN(VCNS)    & 0.9443 & 0.9505 & 0.8660 & 0.8808 & 0.8126 & 0.8460 & \textbf{0.9885} & \textbf{0.9875} & 0.9765 & 0.9779 & 0.9332 & 0.9642 & 0.9034 & 0.9086 \\
		HNHN(TMNS)    & 0.9160 & 0.8840 & 0.8931 & 0.8762 & 0.8645 & 0.8324 & 0.9484 & 0.9387 & 0.9593 & 0.9603 & \underline{0.9717} & \underline{0.9761} & 0.9454 & 0.9529 \\
        HNHN(TCNS)    & 0.7480 & 0.7033 & 0.4699 & 0.4837 & 0.3654 & 0.2629 & 0.9455 & 0.9364 & 0.9103 & 0.9045 & 0.4820 & 0.4977 & 0.8337 & 0.8450 \\
        HNHN(HNS)     & \textbf{0.9633 }& \textbf{0.9601} & \textbf{0.9459} & \textbf{0.9451} & \textbf{0.9472} & \textbf{0.9426 }& 0.9870 & 0.9846 & \textbf{0.9862} & \textbf{0.9852} & \textbf{0.9761} & \textbf{0.9798} & \textbf{0.9847} & \textbf{0.9863} \\
		\midrule
		NHP(SNS)     & 0.9653 & 0.9589 & 0.9156 & 0.9137 & \underline{0.9469} & \underline{0.9414} & 0.9876 & 0.9876 & 0.9665 & 0.9750 & 0.8892 & 0.9238 & \underline{0.9840} & \underline{0.9859}  \\
		NHP(VMNS) 	 & \underline{0.9677} & \underline{0.9628} & 0.9274 & \underline{0.9291} & 0.9258 & 0.9326 & \textbf{0.9974} & \textbf{0.9974} & \underline{0.9740} & \underline{0.9762} & 0.8831 & 0.9146 & 0.9740 & 0.9748 \\
		NHP(VCNS) 	 & 0.9483 & 0.9480 & 0.9048 & 0.9124 & 0.9126 & 0.9240 & \underline{0.9889} & \underline{0.9892} & 0.9719 & 0.9736 & \textbf{0.9667} & \textbf{0.9660} & 0.7284 & 0.7323 \\
		NHP(TMNS)    & 0.8993 & 0.8681 & \underline{0.9355} & 0.9261 & 0.4925 & 0.5252 & 0.9771 & 0.9789 & 0.9587 & 0.9624 & \underline{0.9244} & 0.9128 & 0.9017 & 0.8997 \\
        NHP(TCNS)    & 0.3185 & 0.0702 & 0.3329 & 0.1558 & 0.3880 & 0.2932 & 0.8907 & 0.8921 & 0.8150 & 0.8022 & 0.3405 & 0.1433 & 0.5728 & 0.5521 \\
        NHP(HNS) 	 & \textbf{0.9721} & \textbf{0.9638} & \textbf{0.9467} & \textbf{0.9359} & \textbf{ 0.9473 }& \textbf{0.9415} & 0.9879 & 0.9877 & \textbf{0.9798} & \textbf{0.9779} & 0.9167 & \underline{0.9256} & \textbf{0.9856} & \textbf{0.9867} \\
		\midrule
		HGNNP(SNS)    & \underline{0.9748} & \underline{0.9719} & 0.9146 & \underline{0.9172} & 0.9340 & \textbf{0.9406} & 0.9871 & 0.9863 & 0.9842 & \underline{0.9839} & 0.9421 & \underline{0.9467 }& 0.9594 & 0.9716  \\
		HGNNP(VMNS)   & 0.9623 & 0.9539 & \underline{0.9205} & 0.8886 & \underline{0.9390} & 0.9325 & \underline{0.9917} & \underline{0.9912} & \textbf{0.9861} & \textbf{0.9849} & 0.9368 & 0.9275 & \textbf{0.9777} & \textbf{0.9807}  \\
		HGNNP(VCNS)   & 0.9586 & 0.9605 & 0.8938 & 0.8977 & 0.9208 & 0.9319 & 0.9870 & 0.9864 & \underline{0.9843} & 0.9829 & 0.9368 & 0.9275 & 0.8805 & 0.8850 \\
		HGNNP(TMNS)   & 0.9368 & 0.9127 & 0.8816 & 0.8580 & 0.8751 & 0.8433 & 0.9728 & 0.9708 & 0.9658 & 0.9615 & \textbf{0.9612} & 0.9513 & 0.9635 & 0.9664 \\
        HGNNP(TCNS)   & 0.8108 & 0.7918 & 0.4276 & 0.3815 & 0.3487 & 0.2058 & 0.9723 & 0.9707 & 0.8208 & 0.8354 & 0.3435 & 0.1598 & 0.8342 & 0.8494 \\
        HGNNP(HNS)    & \textbf{0.9855} & \textbf{0.9828} & \textbf{0.9456} & \textbf{0.9308} & \textbf{0.9409} & \underline{0.9354} & \textbf{0.9939} & \textbf{0.9933} & 0.9842 & 0.9834 & \underline{0.9504} & \textbf{0.9550} & \underline{0.9639} & \underline{0.9726}  \\
		\bottomrule
	\end{tabularx}
	\caption{超图链路预测模型性能评估（基于多数据集对比）。本研究比较了四种基线模型（HGNN, HNHN, NHP, HGNNP）在不同负采样策略下的表现，具体包括：SNS、MNS、CNS及本文提出的HNS。对于MNS和CNS两种负样本生成方法，分别在训练集（标记为TMNS, TCNS）和验证集（标记为VMNS, VCNS）上进行了测试。实验覆盖了如CiteSeer、Cora等七个异构信息网络数据集。表中使用加粗与下划线分别标识出最优与次优性能结果。}
	\label{mns_experiment_table}
\end{table}

==> tables/mns_experiment.tex <==
\begin{table}[ht]
	\centering
	\scriptsize
	% \setlength{\tabcolsep}{2pt}
	\begin{tabularx}{0.7\linewidth}{lcccccccr} 
		\toprule
		\Th{Dataset} & \mc{2}{\Th{CiteSeer}} & \mc{2}{\Th{Cora}} & \mc{2}{Pubmed} & \mc{2}{NDC-Class}  \\ 
		& AP & AUC & AP & AUC & AP & AUC & AP & AUC  \\ 
		\midrule
		HGNN      & 0.4869 & 0.4300   & 0.5498 & 0.5377 & 0.641  & 0.6662 & 0.6888  & 0.6717 \\
		HGNN(HNS)    & 0.5208 & 0.5121 & 0.6359 & 0.6096 & 0.6719 & 0.6985 & 0.7161  & 0.7306  \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0339} & \gp{+0.0821} & \gp{+0.0861} & \gp{+0.0719} & \gp{+0.0309} & \gp{+0.0323} & \gp{+0.0273} & \gp{+0.0590} \\
		\midrule
		HNHN        & 0.5627 & 0.5828 & 0.5286 & 0.532  & 0.6156 & 0.6436 & 0.4908  & 0.5322 \\
		HNHN(HNS)    & 0.6323 & 0.6254 & 0.6037 & 0.6236 & 0.6838 & 0.6809 & 0.5280  & 0.5831  \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0696} & \gp{+0.0426} & \gp{+0.0751} & \gp{+0.0916} & \gp{+0.0682} & \gp{+0.0373} & \gp{+0.0372} & \gp{+0.0509} \\
		\midrule
		NHP & 0.5941 & 0.5451 & 0.5481 & 0.549 & 0.5771 & 0.5857 & 0.6017  & 0.6509 \\
		NHP(HNS) & 0.6477 & 0.6496 & 0.637  & 0.627 & 0.6843 & 0.6525 & 0.6997 & 0.7281 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0536} & \gp{+0.1045} & \gp{+0.0889} & \gp{+0.0780} & \gp{+0.1072} & \gp{+0.0668} & \gp{+0.0980} & \gp{+0.0772} \\
		\midrule
		HGNNP         & 0.6359 & 0.6265 & 0.5547 & 0.5553 & 0.6383 & 0.6635 & 0.6022 & 0.6820  \\
		HGNNP(HNS)    & 0.6895 & 0.6975 & 0.6473 & 0.6401 & 0.7055 & 0.6902 & 0.7368  & 0.7657  \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0536} & \gp{+0.071}  & \gp{+0.0926} & \gp{+0.0848} & \gp{+0.0672} & \gp{+0.0267} & \gp{+0.1346} & \gp{+0.0837} \\
		\bottomrule
	\end{tabularx}
    \begin{tabularx}{0.7\linewidth}{lcccccr} 
		\toprule
		\Th{Dataset} & \mc{2}{Email-Enron} & \mc{2}{Human-Disease} & \mc{2}{Plant-Pollinator} \\ 
		& AP & AUC & AP & AUC & AP & AUC \\ 
		\midrule
		HGNN      & 0.8933 & 0.9071 & 0.5772 & 0.5326 & 0.9081 & 0.9287 \\
		HGNN(HNS)    & 0.9068 & 0.918 & 0.6016 & 0.6116 & 0.918 & 0.9315 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0135} & \gp{+0.0109} & \gp{+0.0244} & \gp{+0.079}  & \gp{+0.0099} & \gp{+0.0028} \\
		\midrule
		HNHN        & 0.8712 & 0.8995 & 0.4486 & 0.4169 & 0.9048 & 0.9278 \\
		HNHN(HNS)    & 0.8926 & 0.9077 & 0.5794 & 0.6171 & 0.9054 & 0.9254 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0214} & \gp{+0.0082} & \gp{+0.1308} & \gp{+0.2002} & \gp{+0.0006} & \gn{-0.0024} \\
		\midrule
		NHP & 0.8746 & 0.8899 & 0.5142 & 0.5354 & 0.8635 & 0.9012 \\
		NHP(HNS) & 0.9045 & 0.9019 & 0.695  & 0.6621 & 0.865 & 0.9032 \\
		\rowcolor{LightCyan}
		\tb{Gain} & \gp{+0.0299} & \gp{+0.0120}  & \gp{+0.1808} & \gp{+0.1267} & \gp{+0.0015} & \gp{+0.002}  \\
		\midrule
		HGNNP         & 0.8935 & 0.9123 & 0.5304 & 0.5326 & 0.8685 & 0.8943 \\
		HGNNP(HNS)   & 0.9174 & 0.9196 & 0.5719 & 0.562  & 0.8821 & 0.8968 \\
		\rowcolor{LightCyan}
		\textbf{Gain} & \gp{+0.0239} & \gp{+0.0073} & \gp{+0.0415} & \gp{+0.0294} & \gp{+0.0136} & \gp{+0.0025} \\
		\bottomrule
	\end{tabularx}
	\caption{采用MNS方式生成测试集的负样本，不同模型在不同的负采样方法下的准确率对比.在每种超边预测方法下, 第一行代表使用MNS方法获取负样本, 第二行代表使用HNS方法获取负样本所得到的结果.}
	\label{mns_experiment_table}
\end{table}
